SecFL: Confidential Federated Learning using TEEs

Federated Learning (FL) is an emerging machine learning paradigm that enables multiple clients to jointly train a model to take benefits from diverse datasets from the clients without sharing their local training datasets. FL helps reduce data privacy risks. Unfortunately, FL still exist several issues regarding privacy and security. First, it is possible to leak sensitive information from the shared training parameters. Second, malicious clients can collude with each other to steal data, models from regular clients or corrupt the global training model. To tackle these challenges, we propose SecFL - a confidential federated learning framework that leverages Trusted Execution Environments (TEEs). SecFL performs the global and local training inside TEE enclaves to ensure the confidentiality and integrity of the computations against powerful adversaries with privileged access. SecFL provides a transparent remote attestation mechanism, relying on the remote attestation provided by TEEs, to allow clients to attest the global training computation as well as the local training computation of each other. Thus, all malicious clients can be detected using the remote attestation mechanisms.

==> background.tex <==
%\section{Background}\label{sec:background}

\section{Trusted Execution Environments}
Trusted Execution Environments (TEEs), such as ARM TrustZone~\cite{TrustZone}, Intel SGX~\cite{sgx-explained}, AMD SEV~\cite{SEV}, and Intel TDX~\cite{TDX}, support the design of complex, yet secure, applications. A \gls{tee} is a tamper-resistant processing environment that guarantees the authenticity, the integrity and the confidentiality of its executing code, data and runtime states (e.g., CPU registers, memory and sensitive I/O).
The content of \gls{tee} remains resistant against software attacks even from privileged code, as well as any physical attacks performed on the main memory of the system. In addition, \glspl{tee} offer \emph{attestation} for proving their trustworthiness to third-parties.

\gls{tee} technologies, such as Intel \gls{sgx}, have gained much attention in the industry~\cite{AzureSGX, IBMCloudSGX} as well as in academia~\cite{arnautov2016scone,costan2016intel,tsai2017graphene,shen2020occlum}.
\glspl{tee} can protect cloud-native applications (code and data) not only at rest, in transit, but also during computation (in use) against powerful attackers with privileged access to the underlying system software (\eg{}, the operating system or the hypervisor), as well as, hardware.
To ensure confidentiality and integrity of applications, \glspl{tee} execute their code and data inside an encrypted memory region called \emph{enclave}. 
Adversaries with privileged access cannot read or interfere with the memory region and only the processor can decrypt and execute the application inside an enclave.  

In addition, TEEs such as Intel SGX also provide a mechanism for users to verify that the \gls{tee} is genuine and that an adversary did not alter their application running inside TEE enclaves. The verification process is called \emph{Remote Attestation}~\cite{costan2016intel} and allows users to establish trust in their application running inside an enclave on a remote host.
%Remote attestation is a first step one performs to ensure that an application on a remote host, runs the correct code inside a genuine hardware enclave and it was initialized correctly. After that, the service provider establishes a secure connection to the enclave to transfer secrets and configuration.




==> conclusion.tex <==
\section{Conclusion}
In this paper, we report on our experience with building and deploying \sys,  a secure TensorFlow-based machine learning framework leveraging the hardware-assisted TEEs, specifically Intel SGX.   \sys extends the  security properties of a secure stateless enclave in a single node to secure unmodified distributed stateful machine learning applications. Thereby, it provides a generic platform for end-to-end security for the input data, ML model, and application code. Moreover, it  supports both training and classification phases while providing all three important design properties for the secure machine learning workflow: {\em transparency},  {\em accuracy}, and {\em performance}. \sys is a commercially available platform, and is currently being used in production by four major customers. While there are several open challenges and limitations of our system, our experience shows that \sys strives for a promising approach: it incurs reasonable performance overheads, especially in the classification/inference process, while providing strong security properties against a powerful adversary.  Lastly, we also discussed several open challenges and on-going extensions to the system.



==> figuresTex/fig-sampling-system.tex <==
\begin{figure}[t]
\centering
\includegraphics[scale=0.42]{figuresTex/figures/sampling-system.png}
\caption{Sampling-based approximate computing system.}
\label{fig:sampling-sys}
\end{figure}

==> figuresTex/fig-system-overview.tex <==
\begin{figure}[t]
\centering
\includegraphics[scale=0.42]{figuresTex/figures/system-overview.png}
\caption{System Overview.}
\label{fig:sys-overview}
\end{figure}

==> related.tex <==
\vspace{-2mm}\section{Related work}

In this section, we summarize the related work about secure machine learning and shielded execution using Intel SGX. 

Early works on preserving-privacy data mining techniques have relied on randomizing user data \cite{du2003using, bost2015machine, PrivApprox2017}.
These approaches trade accuracy for privacy. They include a parameter that allows making a trade-off between privacy and accuracy.
The proposed algorithms aim to provide privacy of computation, but they do not protect the results themselves in the cloud, nor do they secure the classification phase. 
%An approach reaching the same accuracy as unprotected variants is to perform machine learning on encrypted data. Bost et al. \cite{bost2015machine} developed protocols to perform privacy-preserving classification. 
While this can protect the users privacy, it does not cover training as in \projectname. Further, we target to provide the same accuracy level as the native execution.
%While this can protect the privacy of the users of a classification service, it does not cover training as in \projectname.

Graepel et al. \cite{graepel2012ml} developed machine learning algorithms to perform both training and classification on encrypted data.
The solution is based on the properties of homomorphic encryption.
%A homomorphic encryption scheme allows operations, such as multiplication and addition, on encrypted data, so that the result can be decrypted by the owner of the private key to yield the same as when performing the operation on the plaintext data. 
However, homomorphic encryption schemes provide restrictive computing operations, and incur high performance overheads. 
There have been a series of recent works~\cite{secureml, gazelle, cryptflow, delphi} aimed to provide secure machine learning platforms with Secure multiparty computation (MPC). Especially, Delphi~\cite{delphi} and CrypTFlow~\cite{cryptflow} demonstrated that they outperform previous works. However, these systems also were designed only for securing inferences.  \projectname is instead based on a hardware-based encryption approach (i.e., Intel SGX) and it supports both training and inference computations.

Shielded execution  provides strong security guarantees for legacy applications running on untrusted platforms~\cite{Baumann2014}. Prominent examples include Haven~\cite{Baumann2014}, SCONE~\cite{arnautov2016scone}, and Graphene-SGX~\cite{tsai2017graphene}.  Our work builds on the SCONE framework.
Intel SGX has become available in clouds~\cite{IBMCloudSGX, AzureSGX}, unleashing a plethora of services to be ported, including Web search~\cite{sgx-websearch},  actor framework~\cite{eactors}, storage~\cite{pesos, speicher}, leases~\cite{t-lease}, monitoring and profilers~\cite{tee-perf,teemon}, software update~\cite{TSR}, FaaS~\cite{clemmys}, networking~\cite{shieldbox, slick}, and data analytics systems~\cite{sgx-pyspark,opaque,Schuster2015}.


%Recently, there has been a significant interest in designing secure data analytics systems based on shielded execution. %For instance, VC3~\cite{Schuster2015} applies SGX to the domain of big data processing by applying it to the Hadoop MapReduce framework. 
%For instance, Opaque~\cite{Opaque} offers distributed secure data analytics on Apache Spark framework using Intel SGX. It reimplements several analytics operators with C++ to run them inside enclaves. Thus, it does not support all operators as native Apache Spark. 
%In addition, it requires to run Spark driver at a trusted domain which might affect the performance of analytics computations because of the high latency communication between driver and workers. 
%SGX-Pyspark~\cite{sgx-pyspark} overcomes these problems by running python operations of PySpark framework inside SGX enclaves. However, this system was not tested with machine learning workloads. 

%The work from Ohrimenko et al.~\cite{ohrimenko} is the most relevant for \projectname, where they leveraged Intel SGX to secure specific machine learning operators. In contrast to work  from Ohrimenko et al.~\cite{ohrimenko}, we present the first generic machine learning framework based on the widely-used TensorFlow framework, which can support a wide-range of unmodified existing TensorFlow applications. 

Recently, several secure machine learning systems have been proposed, which rely on Intel SGX to support secure machine learning~\cite{privado, slalom, chiron, ohrimenko}. 
%However, these systems were designed for secure inferences only. 
Privado~\cite{privado} proposes a mechanism to obtain oblivious neural networks. Then, it executes the oblivious neural network inside SGX enclaves for secure inferencing.  Slalom~\cite{slalom} makes use of a combination of Intel SGX and untrusted GPUs to secure Deep Neural Networks (DNNs) computations. The idea of Slalom is that it splits the DNN computations into linear operations (e.g., matrix multiplications) on GPUs, whereas performing the non-linear operations  (eg. ReLUs operations) inside Intel SGX enclaves. This approach allows achieving much better performance since the intensive computation is performed with GPUs. Unfortunately, Slalom still has several limitations. First, as Privado, it focuses only on secure inferences. It refers to secure training computations as a research challenge. Second, It requires Tensorflow users to heavily modify or redevelop their existing code. Third, it does not support distributed settings, i.e., it does not support secure connections between SGX enclaves. Finally, Slalom is not production ready, in fact, it indicates that it can be used only for testing. 
Chiron~\cite{chiron} is the most relevant for \projectname, where they leveraged Intel SGX for privacy-preserving machine learning services. Unfortunately, Chiron is a single-threaded system within an enclave. In addition, Chiron requires adding an interpreter and model compiler into enclaves which introduce significant runtime overhead since the limited EPC size.  The work from Ohrimenko et al.~\cite{ohrimenko} also used Intel SGX to secure machine learning computations, however, it supports only a limited number of operators.  In contrast, we propose \projectname~ --- a practical distributed machine learning framework for securing both training and inference computations. 
%In contrast to work  from Ohrimenko et al.~\cite{ohrimenko}, we present the first generic machine learning framework based on the widely-used TensorFlow framework, which can support a wide-range of unmodified existing TensorFlow applications. 
%We built \projectname based on the widely-used TensorFlow framework, which can support a wide-range of unmodified existing TensorFlow applications. 

%In this work, we propose \projectname --- a practical distributed framework for securing both training and inference deep neural network computations over sensitive input data. 
%In contrast to work  from Ohrimenko et al.~\cite{ohrimenko}, we present the first generic machine learning framework based on the widely-used TensorFlow framework, which can support a wide-range of unmodified existing TensorFlow applications. 

%Currently, \projectname  does not make use of GPUs to deploy TensorFlow operators since they do not provide a TEE. In this space, Graviton~\cite{graviton} recently proposed hardware extensions to provide a secure  environment on GPUs. We plan to leverage Graviton's extensions for deploying \projectname applications on GPUs. 

